Robotized Ultrasound Imaging of the Peripheral Arteries -- a Phantom Study

The first choice in diagnostic imaging for patients suffering from peripheral arterial disease is 2D ultrasound (US). However, for a proper imaging process, a skilled and experienced sonographer is required. Additionally, it is a highly user-dependent operation. A robotized US system that autonomously scans the peripheral arteries has the potential to overcome these limitations. In this work, we extend a previously proposed system by a hierarchical image analysis pipeline based on convolutional neural networks in order to control the robot. The system was evaluated by checking its feasibility to keep the vessel lumen of a leg phantom within the US image while scanning along the artery. In 100 % of the images acquired during the scan process the whole vessel lumen was visible. While defining an insensitivity margin of 2.74 mm, the mean absolute distance between vessel center and the horizontal image center line was 2.47 mm and 3.90 mm for an easy and complex scenario, respectively. In conclusion, this system presents the basis for fully automatized peripheral artery imaging in humans using a radiation-free approach.

==> README <==
                 The dgruyter package:                 
preparing books and journals for Walter de Gruyter GmbH


File:       README
Author:     le-tex publishing services


DESCRIPTION
===========

The dgruyter package assists in preparing manuscripts for de Gruyter
with {\LaTeX}. It provides some special commands for journal papers
as well as for books and generates the required appearance.
Together with corresponding font packages it allows to produce the 
final layout of De Gruyter books and journal articles.

Copyright:  (C) 2015, 2016, 2017 Walter de Gruyter GmbH


FILES IN DISTRIBUTION
=====================

   BASE DISTRIBUTION:

      README                  This file.
      dgruyter.ins            Package installation file.
      dgruyter.dtx            Package source file.
      dg-degruyter.eps/.pdf   Logo files.
      dg-mouton.eps/.pdf      Logo files.
      dg-saur.eps/.pdf        Logo files.
      DG_attention.eps/.pdf   Vignette files.
      DG_exercise.eps/.pdf    Vignette files.
      DG_information.eps/.pdf Vignette files.
      DG_notice.eps/.pdf      Vignette files.
      DG_question.eps/.pdf    Vignette files.
      book.tex                Template file for a book.
      article.tex             Template file for a journal article.
      issuetoc.tex            Template file for a journal issue toc.


   DOCUMENTATION:

      dgruyter.pdf            User manual for dgruyter package. 
                              It is produced as described below.


BASIC INSTALLATION
====================

   To get the package style file 'dgruyter.sty' and the
   index style files 'dgruyter.ist' and 'dgruyter.xdy' execute:
     latex dgruyter.ins

   The minimum requirement to use the package is to have
     dgruyter.sty and dgruyter.ist/dgruyter.xdy
     (as well as the logo and vignette files)
     in a directory where TeX can find it.

   To get the documentation 'dgruyter.pdf' execute:
     pdflatex dgruyter.dtx (at least twice)

